Vox-E: Text-guided Voxel Editing of 3D Objects

Large scale text-guided diffusion models have garnered significant attention due to their ability to synthesize diverse images that convey complex visual concepts. This generative power has more recently been leveraged to perform text-to-3D synthesis. In this work, we present a technique that harnesses the power of latent diffusion models for editing existing 3D objects. Our method takes oriented 2D images of a 3D object as input and learns a grid-based volumetric representation of it. To guide the volumetric representation to conform to a target text prompt, we follow unconditional text-to-3D methods and optimize a Score Distillation Sampling (SDS) loss. However, we observe that combining this diffusion-guided loss with an image-based regularization loss that encourages the representation not to deviate too strongly from the input object is challenging, as it requires achieving two conflicting goals while viewing only structure-and-appearance coupled 2D projections. Thus, we introduce a novel volumetric regularization loss that operates directly in 3D space, utilizing the explicit nature of our 3D representation to enforce correlation between the global structure of the original and edited object. Furthermore, we present a technique that optimizes cross-attention volumetric grids to refine the spatial extent of the edits. Extensive experiments and comparisons demonstrate the effectiveness of our approach in creating a myriad of edits which cannot be achieved by prior works.

==> figures/comparisons_dff.tex <==
\begin{figure} %
\centering
%\rotatebox{90}{DFF + CLIP-NeRF}
\jsubfig{\includegraphics[height=1.97cm, trim={1.0cm 3.0cm 2.5cm 1.0cm}, clip]{images/comparisons/dff/horse_wood.png}} {\footnotesize {``A wood carving of a horse"}}\hfill
\jsubfig{\includegraphics[height=1.97cm, trim={1.0cm 3.0cm 2.5cm 1.0cm}, clip]{images/comparisons/dff/horse_hat.png}} {\footnotesize {``Horse wearing a santa hat"}}\hfill
\jsubfig{\includegraphics[height=1.97cm, trim={1.0cm 3.0cm 2.5cm 1.0cm}, clip]{images/comparisons/dff/horse_donkey.png}}{\footnotesize {``A donkey"}}\hfill
\jsubfig{\includegraphics[height=1.97cm, trim={1.0cm 3.0cm 2.5cm 1.0cm}, clip]{images/comparisons/dff/horse_carousel.png}}
{\footnotesize {``A carousel horse"}}
\vspace{5pt} 
\caption{\textbf{Comparison to DFF combined with CLIP-NeRF}. As illustrated above, this method is only suited for appearance modifications (such as "A wood carving of a horse"), and therefore does not succeed in editing with prompts that require geometric modifications to the object (such as "A donkey" and "Horse wearing a santa hat"). 
}
\label{fig:comparisonsdff}
\end{figure}


==> figures/qualatative_results.tex <==
\twocolumn[{%
	\renewcommand\twocolumn[1][]{#1}%
	\maketitle
 \vspace{-25pt}
	\begin{center}
%\begin{figure*}[h]
%        \centering
        \setlength{\tabcolsep}{2pt}
        \begin{tabular}{cc ccc cc cc ccc}
        
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/dog_orig.png} &
        { } &
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/20_glasses_dog.png} & 
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/0_glasses_dog.png} & 
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/140_glasses_dog.png} &
        %
        {  } &

        { } &
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/20_yarn_dog.png} & 
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/0_yarn_dog.png} & 
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/140_yarn_dog.png} \\
        %
        Original
        && \multicolumn{3}{c}{``A render of a light grey dog \emph{wearing big glasses}''} &
        && \multicolumn{3}{c}{``A render of a \emph{yarn doll} of a light grey dog''} \\
        %
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/cat_orig.png} &
        { } &
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/20_glasses_cat.png} & 
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/0_glasses_cat.png} & 
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/140_glasses_cat.png} &
        %
        { } &

        { } &
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/20_yarn_cat.png} & 
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/0_yarn_cat.png} & 
        \includegraphics[width=0.12\textwidth,trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{images/teaser/teaser_abra/140_yarn_cat.png} \\
        %
        Original
        && \multicolumn{3}{c}{``A render of a ginger cat \emph{wearing big glasses}''} &
        && \multicolumn{3}{c}{``A render of a \emph{yarn doll} of a ginger cat''} \\
        Original
        && \multicolumn{3}{c}{\he{``A render of a $\left<object\right>$ \emph{wearing big glasses}''}} &
        && \multicolumn{3}{c}{\he{``A render of a \emph{yarn doll} of a $\left<object\right>$''}} \\
        %
        %
    \end{tabular}
    \vspace{1mm}
    \captionof{figure}{Given multiview images of an object (left), our technique enables generating volumetric edits from text prompts.  
    The objects can be edited either \emph{locally} (center) or \emph{globally} (right), depending on the nature of the user-provided text prompt. Our edits may incorporate significant geometric and appearance changes, while faithfully preserving  the input object. \hec{consider having a single prompt on bottom and explaining in the caption that we use simple prompts that contain only the category of the object (e.g., cat or dog in the examples above) and the desired edit. } \hec{I trimmed the images too much, maybe consider using models that (unlike the cat) don't have such a long tail, or maybe just a slightly different viewpoint}
    }
    \label{fig:teaser}
	\end{center}
%\end{figure*}        
}]


==> figures/real_scenes.tex <==
\begin{figure} %
\centering
\rotatebox{90}{\whitetxt{xxx}Input} \hfill
\jsubfig{\includegraphics[height=1.9cm]{images/real_scenes/flowers/flowers_input.png}}{} \hfill
\jsubfig{\includegraphics[height=1.9cm]{images/real_scenes/new/pinecone_input_fig5.png}}{} \hfill
\jsubfig{\includegraphics[height=1.9cm]{images/real_scenes/pinecone/pinecone_input.png}}{} \vspace{1.5pt} 
\\ 
\rotatebox{90}{\whitetxt{xxx}Initial} \hspace{0.5pt}
\jsubfig{\includegraphics[height=1.9cm]{images/real_scenes/new/dvgo_flower_init.png}}{} \hfill
\jsubfig{\includegraphics[height=1.9cm]{images/real_scenes/new/pinecone_recon_fig5.png}}{} \hfill
\jsubfig{\includegraphics[height=1.9cm]{images/real_scenes/new/dvgo_recon.png}}{} \vspace{1.5pt} 
\\ 
\rotatebox{90}{\whitetxt{xxx}Edited} \hfill
\jsubfig{\includegraphics[height=1.9cm]{images/real_scenes/new/dvgo_sunflowers.png}}{\footnotesize {``A vase with sunflowers"}}\hfill
\jsubfig{\includegraphics[height=1.9cm]{images/real_scenes/new/pineapple_fig5.png}}{\footnotesize {``A pineapple on the ground"}}\hfill
\jsubfig{\includegraphics[height=1.9cm]{images/real_scenes/new/dvgo_pond.png}}{\footnotesize {``A pinecone floating in a pond"}}
\vspace{1.5pt}
\caption{Qualitative results of our method on the publicly available $360^\circ$ \emph{Real Scenes} \cite{mildenhall2021nerf}. We show images rendered from the initial grid in the middle row and from the our edited grid in the bottom row. As illustrated above, our method can generate convincing edits on these real scenes without explicitly modeling the foreground and background regions. 
 }
\label{fig:realscenes}
\end{figure}


==> figures/supp_attn_duck.tex <==
\begin{figure*} %
\centering
\rotatebox{90}{\whitetxt{xxx}2D Edit}
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/2d_edit/0_edit.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/2d_edit/30_edit.png}}{} \hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/2d_edit/60_edit.png}}{} \hfil
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/2d_edit/90_edit.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/2d_edit/120_edit.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/2d_edit/150_edit.png}}{}
\rotatebox{90}{\whitetxt{xxx}3D Edit}
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/3d_edit/0.png}}{} \hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/3d_edit/30.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/3d_edit/60.png}}{} \hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/3d_edit/90.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/3d_edit/120.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/3d_edit/150.png}}{}
\rotatebox{90}{\whitetxt{xxx}2D Object}
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/2d_object/0_object.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/2d_object/30_object.png}}{} \hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/2d_object/60_object.png}}{} \hfil
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/2d_object/90_object.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/2d_object/120_object.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/2d_object/150_object.png}}{}
\rotatebox{90}{\whitetxt{xxx}3D Object}
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/3d_object/0.png}}{} \hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/3d_object/30.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/3d_object/60.png}}{} \hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/3d_object/90.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/3d_object/120.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/3d_object/150.png}}{}
\rotatebox{90}{\whitetxt{xxx}Blend Edit}
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/blend_edit/0.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/blend_edit/30.png}}{} \hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/blend_edit/60.png}}{} \hfil
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/blend_edit/90.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/blend_edit/120.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/blend_edit/150.png}}{}
\rotatebox{90}{\whitetxt{xxx}Blend Object}
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/blend_object/0.png}}{} \hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/blend_object/30.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/blend_object/60.png}}{} \hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/blend_object/90.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/blend_object/120.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/blend_object/150.png}}{}
\rotatebox{90}{\whitetxt{xxx}Output}
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/output/0.png}}{} \hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/output/30.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/output/60.png}}{} \hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/output/90.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/output/120.png}}{}\hfill
\jsubfig{\includegraphics[height=2.78cm]{images/supp_attn/duck/output/150.png}}{}
\vspace{5pt} 
\caption{\textbf{Visualizing 360 degrees of 3d cross-attention grids and the 2D cross-attention maps used for supervision}.  We visualize the trained 3d cross-attention grids and the corresponding 2D cross-attention maps used as training supervision for the edit region "hat" (top two rows) and the object region "duck" (rows 3 and 4). We also add a blended image of the 3d attention grid and the pre-refinement edit grid for both edit (row 5) and object (row 6) regions. The bottom row shows the output edit.
}
\label{fig:supp_attn}
\end{figure*}
